Optimal Gradient-based Algorithms for Non-concave Bandit Optimization

Bandit problems with linear or concave reward have been extensively studied, but relatively few works have studied bandits with non-concave reward. This work considers a large family of bandit problems where the unknown underlying reward function is non-concave, including the low-rank generalized linear bandit problems and two-layer neural network with polynomial activation bandit problem. For the low-rank generalized linear bandit problem, we provide a minimax-optimal algorithm in the dimension, refuting both conjectures in [LMT21, JWWN19]. Our algorithms are based on a unified zeroth-order optimization paradigm that applies in great generality and attains optimal rates in several structured polynomial settings (in the dimension). We further demonstrate the applicability of our algorithms in RL in the generative model setting, resulting in improved sample complexity over prior approaches. Finally, we show that the standard optimistic algorithms (e.g., UCB) are sub-optimal by dimension factors. In the neural net setting (with polynomial activation functions) with noiseless reward, we provide a bandit algorithm with sample complexity equal to the intrinsic algebraic dimension. Again, we show that optimistic approaches have worse sample complexity, polynomial in the extrinsic dimension (which could be exponentially worse in the polynomial degree).

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Our abstract and introduction accurately reflect our main contribution, which is also summarized in Table \ref{tbl:main}. }
  \item Did you describe the limitations of your work?
    \answerYes{In the Preliminary section we clearly state the settings we considered and when our results apply. }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Our work is theoretical and generally will not have negative social impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{The assumptions are clearly included in every theorem or lemma. }
    \item Did you include complete proofs of all theoretical results?
    \answerYes{All the proofs can be found in the appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/intro2.tex <==
\section{Introduction}

Bandits are a class of online decision making problems where an agent interacts with the environment and aims to learn the optimal reward it can get. It is also a simplified version of Reinforcement Learning (RL) problems. In many real world applications, bandit and RL problems are characterized with big or infinite (or continuous) action space. Then to encode the reward information associated with the action, function approximation for the reward function are proposed, with the simplest settings being the linear bandits~\citep{abbasi2011improved}.
Stochastic linear bandits assume the mean reward to be the inner product between the unknown model parameter and the feature vector associated with the action. This setting has received extensive studies, and people have derived algorithms with sample complexity matching the lower bound~\citep{lattimore2020bandit,filippi2010parametric,abbasi2011improved,bubeck2012regret}.
This is not surprising since there is no benefit of using adaptive algorithms in terms of PAC risk. Even some non-adaptive matrix sensing algorithms can achieve optimal PAC risk \citep{mannor2004sample}.

However, linear bandits suffer from the limited power of representing the reward function in the complex reality. To take a step further beyond the linear setting, it becomes more challenging to understand the optimal learning rates. Unlike linear bandits, more sophisticated adaptive algorithms become necessary. For instance, a natural first step is to look at quadratic~\citep{katariya2017stochastic} and higher-order polynomials~\citep{hao2020low}. In the context of phase retrieval, which is a special case for the quadratic bandit, people have derived algorithms that achieve minimax risks among non-adaptive algorithms \citep{arias2012fundamental,lecue2013minimax,cai2016optimal}. However, it doesn't match our lower bound among all adaptive algorithms on the dependence of problem dimension. 

==> sections/setting.tex <==
\section{The Settings}
